Experiments in Verification of Linear Model Predictive Control: Automatic Generation and Formal Verification of an Interior Point Method Algorithm

Classical control of cyber-physical systems used to rely on basic linear controllers. These controllers provided a safe and robust behavior but lack the ability to perform more complex controls such as aggressive maneuvering or performing fuel-efficient controls. Another approach called optimal control is capable of computing such difficult trajectories but lacks the ability to adapt to dynamic changes in the environment. In both cases, the control was designed offline, relying on more or less complex algorithms to find the appropriate parameters. More recent kinds of approaches such as Linear Model-Predictive Control (MPC) rely on the online use of convex optimization to compute the best control at each sample time. In these settings, optimization algorithms are specialized for the specific control problem and embed on the device. This paper proposes to revisit the code generation of an interior point method (IPM)algorithm, an efficient family of convex optimization, focusing on the proof of its implementation at code level. Our approach relies on the code specialization phase to produce additional annotations formalizing the intented specification of the algorithm. Deductive methods are then used to prove automatically the validity of these assertions. Since the algorithm is complex, additional lemmas are also produced, allowing the complete proofto be checked by SMT solvers only. This work is the first to address the effective formal proof of an IPM algorithm. Theapproach could also be generalized more systematically to code generation frameworks, producing proof certificate along the code, for numerical intensive software.

==> 4-annotation.tex <==
\section{Automatic annotation of the code}
\label{sec:annot}

The code is prepared to ease its proof but the specification still remains to be
formalized as function contracts, describing the computation of an
$\epsilon$-optimal solution. This requires to enrich ACSL with some new
mathematics definitions. We introduce a set of axiomatic definition to specify
optimization related properties. These definitions require, in turn, additional
concepts related to matrices. Similar approaches were already
proposed~\cite{nfm12_2} but were too specific to ellipsoid problems. We present
here both the main annotation and the function local contracts, which ease the global
proof.

\paragraph{Matrix axiomatic.}
To write the mathematics property, we need to be able to express
the notion of Matrix and operations over it. Therefore we defined a new ACSL
axiomatic. An ACSL axiomatic permits the specifier to extend the ACSL language with new
types and operators, acting as an algebraic specification.

\begin{lstlisting}[style=acsl, frame=TL]
axiomatic matrix
{
	type LMat;
\end{lstlisting}

First, we defined the new type: \code{LMat} standing for Logic Matrix.
This type is abstract therefore it will be defined by its operators.
	
\begin{lstlisting}[style=acsl, frame=L]
       // Getters
	logic integer getM(LMat A);
	logic integer getN(LMat A);
	logic real mat_get(LMat A, integer i, integer j);
        // Constructors
	logic LMat MatVar(double* ar, integer m, integer n) reads ar[0..(m*n)];
	logic LMat MatCst_1_1(real x0);
	logic LMat MatCst_2_3(real x0, real x1, real x2, real x3, real x4, real x5);
\end{lstlisting}

Getters allow to extract information from the type while constructors bind new
\code{LMat} object.
The first constructor is followed by a \code{read} clause stating which
part of the memory affects the corresponding \code{LMat} object. The Constant
constructor take directly the element of the matrix as argument, it can be
replaced with an ACSL array for bigger matrix sizes.


\begin{lstlisting}[style=acsl, frame=L]
	logic LMat mat_add(LMat A, LMat B);
	logic LMat mat_mult(LMat A, LMat B);
	logic LMat transpose(LMat A);
	logic LMat inv(LMat A);
	...
\end{lstlisting}


Then the theory defined the operations on the \code{LMat} type.
These are defined axiomatically, with numerous axioms to cover their various
behavior. We only give here a excerpt from that library.

\begin{lstlisting}[style=acsl, frame=BL]
	axiom getM_add:	\forall LMat A, B; getM(mat_add(A, B))==getM(A);
	axiom mat_eq_def:
	\forall LMat A, B;
		(getM(A)==getM(B))==> (getN(A)==getN(B))==>
		(\forall integer i, j; 0<=i<getM(A) ==> 0<=j<getN(A) ==>
			mat_get(A,i,j)==(mat_get(B,i,j))==>
			A == B;
	...
}
\end{lstlisting}

\paragraph{Matrix operations.}

As explained in previous Section, the matrix computation are encapsulated into
smaller functions. Their contract states the equality between the resulting
matrix and the operation computed. The extensionality axiom (\code{mat\_eq\_def})
is required to prove this kind of contract. Extensionality means that if two
objects have the same external properties then they are equal.

\begin{figure}
%\vspace{-1em}
\begin{lstlisting}[style=acsl]
assert getM(MatVar(dX,2,1)) == 2;
assert getN(MatVar(dX,2,1)) == 1;
assert getM(MatVar(cholesky,2,1)) == 2;
assert getN(MatVar(cholesky,2,1)) == 1;
assert mat_get(MatVar(dX,2,1),0,0) == mat_get(\old(mat_scal(MatVar(cholesky,2,1),-1.0)),0,0);
assert mat_get(MatVar(dX, 2, 1),1,0) == mat_get(\old(mat_scal(MatVar(cholesky,2,1),-1.0)),1,0);
\end{lstlisting}
\caption{Assertion appended to the function of Figure \ref{fig:mat_op}}
\label{fig:mat_op_assert}
%\vspace{-1em}
\end{figure}

This axiom belong to the matrix axiomatic but is too general to be used therefore
lemmas specific to the matrices size are added for each matrix affectation.
This lemma can be proven with the previous axioms and therefore does not introduce
more assumption.

The proof remains difficult or hardly automatic for SMT solvers therefore we
append additional assertions, as sketched in Figure~\ref{fig:mat_op_assert}, at
then end of function stating all the hypothesis of the extensionality lemma.
Proving these post-conditions is straightforward and smaller goals need now to be proven.

Further split of functions into smaller functions is performed when functions
become larger.%The refinement process is further developed when functions become large. 
As an example, for operations on matrices of size $m^2$, there is $m^2$ lines of C code 
manipulating arrays and logic. To avoid large goals involving array accesses for SMT solvers when $m$ becomes greater than $10$,
  each operation is encapsulated as a separate function annotated by the operation on a single element:

\begin{lstlisting}[style=acsl]
mat_get(MatVar(dX,2,1),0,0) == mat_get(\old(mat_scal(MatVar(cholesky,2,1),-1.0)),0,0);
\end{lstlisting}

These generated goals are small enough for SMT. The post-condition of the
matrix operation remains large but the array accesses are abstracted away by all the
function call and therefore becomes provable by SMT solvers.

\paragraph{Optimization axiomatic.}
Besides generic matrix operators, we also need some operators specific to our
algorithm. The Newton step defined in Eq.  \eqref{eq:dX} as well as the local
norm of Eq.~\eqref{eq:norm} are both based on the gradient and the Hessian of
the barrier function (Eq.~\ref{eq:bf}) encoding the feasible set. These
functions are then defined by the matrix $A$, the vector $b$ and the local point
$X$.


\begin{lstlisting}[style=acsl, frame=TL]
axiomatic Optim
{
	logic LMat hess(LMat A, LMat b, LMat X);
	logic LMat grad(LMat A, LMat b, LMat X);
\end{lstlisting}

Hessian and gradient are hard to define without real analysis which
is well beyond the scope of this article. Therefore we decided to directly axiomatize
some theorems relying on their definition like \cite[Th4.1.14]{nesterov94}.
%TODO: Ecrire le théorème pourrait etre bien

\begin{lstlisting}[style=acsl, frame=L]
	logic real sol(LMat A, LMat b, LMat c);
\end{lstlisting}

The \code{sol} operator represents $x^*$, the exact solution which can be
defined by the following property:

\begin{myprop}[Axiomatic characterization of Definition \ref{def:lp_sol} (Eqs~\eqref{eq:feasible_set}--\eqref{eq:opt_pt})]
$s$ is a solution of Eq.~\eqref{eq:lin_pb} if and only if
\begin{enumerate}
\item For all $y \in E_f$, $c^T y \geq s$
\item For all $y \in \mathbb{R}$, $\forall x \in E_f, c^T x \geq y$ implies $s \geq y$
\end{enumerate}
\end{myprop}

An ACSL equivalent definition is:

\begin{lstlisting}[style=acsl, frame=L]
logic real sol(LMat A, LMat b, LMat c);
axiom sol_min: \forall LMat A, b, c;
	\forall LMat y; mat_gt(mat_mult(A, y), b) ==>
		dot(c, y) >= sol(A, b, c);
axiom sol_greater: \forall LMat A, b, c;
	\forall Real y;
		(\forall LMat x; mat_gt(mat_mult(A, x), b) ==> dot(c, x) >= y) ==>
			sol(A, b, c) >= y;
\end{lstlisting}

Then we defined some operators representing definitions \ref{def:norm}, \ref{def:acc} and \textsc{Lower}\eqref{eq:lower}.

\begin{lstlisting}[style=acsl, frame=BL]
	logic real norm(LMat A, LMat b, LMat x, LMat X) =
		\sqrt(mat_get(mat_mult(transpose(x), mat_mult(inv(hess(A, b, X)), x)), (0), (0)));
	logic boolean acc(LMat A, LMat b, LMat c, real t, LMat X, real beta) =
		((norm(A, b, mat_add(grad(A, b, X), mat_scal(c, t)), X))<=(beta));
	...
}
\end{lstlisting}

\paragraph{Contract on \code{pathfollowing}.}

A sound algorithm must produce a point in the feasible set such that
its cost is $\epsilon$-close to $sol$. This represents the functional
specification
that we expect from the code and is asserted by two post-conditions:

%TODO: Peut etre enelever les barres:
\begin{lstlisting}[style=acsl, frame=L]
ensures mat_gt(mat_mult(A, MatVar(X, N, 1)), b);
ensures dot(MatVar(X, 2, 1), c) - sol(A, b, c) < EPSILON
\end{lstlisting}

as well as two preconditions stating that $X$ is feasible and close enough to the analytic center:
\begin{lstlisting}[style=acsl, frame=L]
requires mat_gt(mat_mult(A, MatVar(X, N, 1)), b);
requires acc(A, b, c, 0, MatVar(X, N, 1), BETA);
\end{lstlisting}

Thanks to our two new theories \code{Matrix} and \code{Optim}, writing and reading this
contract is straightforward and can be checked by anyone familiar with linear programming. 
%Most of our work consists in proving this annotation by
%expressing other annotations disseminate on the whole code and proving
%all of them.
Our contribution focuses on the expression on intermediate annotations, spread over the code, to 
support the overall proof of specifications.

\paragraph{Main Loop.}

A loop needs to be annotated by an invariant to have its Weakest precondition
computed. We need three invariant for our pathfollowing algorithm.
The first one guarantees the feasibility of $X$ while the second one
states the conservation of the $ACC$ (cf. Def.~\ref{def:acc})
The third invariant assert that $t$ is increasing enough on each iteration, more
specifically that it is greater than a geometric progression\eqref{eq:lower}.

\begin{lstlisting}[style=cacsl]
/*@ loop-invariant mat_gt(mat_mult(A, MatVar(X, N, 1)), b);
  @ loop-invariant acc(A, b, c, t, MatVar(X, N, 1), BETA);
  @ loop-invariant t > lower(l);*/
for (int l = 0; l < NBR;l++) { ... }
\end{lstlisting}

Proving the initialization is straightforward, thanks to the main preconditions.

We wrote one ACSL lemma for each invariant. Whenever it is possible we try
to follow \cite{nesterov94}, for example by translating \cite[Th4.1.5]{nesterov94} and Theorem \ref{th:acc}.

The last two loop invariant are combined to prove the second post-condition of \code{pathfollowing}
thanks to Theorem \ref{th:main}. \code{NBR} is computed from $k_{last}$.

\begin{myth}\label{th:main}\cite[Th4.2.7]{nesterov94}
Let $t \geq 0$, and $X$ such that $ACC(X, t, \beta)$ then
\begin{equation}
c^T X - c^T X^* < \frac{1}{t} \times (1 + \frac{(\beta + 1)\beta}{1 - \beta})
\end{equation}
\end{myth}

\paragraph{Loop body.}

In the main loop there are three function calls: \code{update\_pre} computing some common
values, \code{update\_t} and \code{update\_x}(Figure \ref{fig:calltree}). Therefore Theorem
\ref{th:acc} is broken into several properties and the corresponding post-conditions.
For example, the contract of \code{update\_t} is:

\begin{lstlisting}[style=cacsl]
/*@ requires MatVar(hess, N, N)==hess(A, b, MatVar(X, N, 1));
  @ requires acc(A, b, c, t, MatVar(X, N, 1), BETA);
  @ ensures  acc(A, b, c, t, MatVar(X, N, 1), BETA + GAMMA);
  @ ensures t > \old(t)*(1 + GAMMA/(1 + BETA));*/
void update_t();
\end{lstlisting}

The first post-condition is an intermediary results stating that:

\begin{equation}\label{eq:update_t_ensures_1}
ACC(X, t+dt, \beta + \gamma)
\end{equation}

This result is used as precondition
for \code{update\_x}.
The second precondition corresponds to the product of $t$ by the common ratio of the
geometric progression $\textsc{Lower},$ cf. \eqref{eq:lower}
which will be used to prove the second invariant of the loop.
The first precondition is a post-condition from \code{update\_pre} and the second
one is the first loop invariant.

The verification is performed thanks to two sets of axioms we developed, supporting 
(1) the definition of matrices in ACSL or (2) defining properties of operators in linear programming.
While the first set describing matrices commutation or norm positivity could be proved, it is an additional
work outside of the scope of our contribution. The second set is more challenging to prove and corresponds
to the axiomatization of some theorems from \cite{nesterov94}. Their definition as axioms was carefully
addressed and the number of such axioms minimized. 
Proving this second set would be interesting to prove but using the \textsf{Frama-C} framework 
might not be the best solution.

%We had to write diffrent kinds of axioms, most of them are required to define matrices in
%ACSL or operators require for linear programming. This axioms can't be removed so you have
%to be really careful to them. The other axioms are of two kinds, the first are direct
%results about matrices like commutation, norm positivity... This results are not axiomed
%and could be proved from the definition. We decided to let them as axioms since it was not
%a real challenge to prove. Last but not least we axiomatize some theorem from \cite{nesterov94}.
%We were really carefult when we choose them and tried to reduce as much as possible their number.
%This axioms would be interesting to prove but using the Frama-C framework might not be the best
%solution.

All this axioms are potential flaws for the verification. One solution is to translate
them within a Theorem prover such as \textsf{Coq}\cite{Bertot2004} and proving them instead of assuming them.
This represent a certain amount of work but translating the matrices to a theorem prover would also
have the advantage to check the matrix axiomatic we wrote. This could be done by providing
a bijection between the translation of our matrices and matrices defined in \textsf{Coq}
libraries like \textsf{SSReflect}\cite{ssreflect}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "00-main"
%%% End:

